Table-LLM-Specialist: Language Model Specialists for Tables using Iterative Generator-Validator Fine-tuning

Language models such as GPT and Llama have shown remarkable ability on diverse natural language tasks, yet their performance on complex table tasks (e.g., NL-to-Code and data cleaning) remains suboptimal. Improving performance typically requires task-specific fine-tuning, which depends on expensive human labeling and is prone to overfitting. In this work, we propose Table-LLM-Specialist, a self-trained fine-tuning paradigm designed for table tasks. Our key insight is that many table tasks admit two dual formulations: a generative version and a classification version. Leveraging this duality, we introduce a Generator-Validator paradigm that iteratively generates and validates training data using language models, enabling effective fine-tuning without manually labeled data. Extensive evaluations on Llama, GPT-3.5, and GPT-4 show that Table-LLM-Specialist achieves (1) strong performance across diverse tasks compared to base models, for example, models fine-tuned on GPT-3.5 often surpass GPT-4 level quality; (2) lower deployment cost by enabling smaller models to reach high quality with reduced latency and cost; and (3) better generalization across multiple benchmarks, due to training on diverse, systematically generated data from real-world tables. Our code is available at https://github.com/microsoft/Table-Specialist. Models fine-tuned with Table-LLM-Specialist have been integrated into Microsoft Excel and are deployed in production for automated table data cleaning.

==> sections/Prompts/error_detection_generation.tex <==
Instruction:
# Task Description: Given the table column <Column> below, please brainstorm an erroneous cell <CELL> that is NOT compatible with the <Column>, which if added to the <Column>, would be considered as a data error.

For example:
(1) When the <Column> has a list of string-valued names, an error <CELL> can be a number as a special placeholder such as "99999" or "0". 
(2) When the <Column> has a list of numbers, an error <CELL> can be is a string.
(3) An error <CELL> can also be placeholder punctuation like "?", "!", "***" and "--"
(4) An error <CELL> can also be of a semantic type that is obviously not compatible with the rest of the  <Column>, e.g., <CELL> is an email address while the  <Column> has a list of URLs, or <CELL> is a phone number while <Column> has a list of countries, etc.

Please brainstorm an **ERROR** cell <CELL>  **NOT** compatible with the <Column>. 

**DO** generate <CELL> using realistic strings
** NEVER ** generate fake <CELL> like "123 Main Street".
** NEVER ** generate fake <CELL> like "123456789"
** NEVER ** generate fake <CELL> like "12345"
** NEVER ** generate fake <CELL> like "ABC"
** NEVER ** generate fake <CELL> like "ABCD"
** NEVER ** generate fake <CELL> like "john.doe@example.com"

Return a JSON in the format {"ERROR": "<CELL>"}.

------

## Input:


|11:43.1|
|10:30.1|
|10:54.7|
|23:03.1|
|11:01|
|11:27.4|
|08:24.6|
|13:44.4|


## Output:

{"ERROR": "new zealand"}


------

## Input:


|Mens 100m butterfly|
|Womens 100m freestyle|
|Mens 200m breaststroke|
|Womens 200m backstroke|


## Output:

{"ERROR": "Olivia.Mcbath@gmail.com"}


------


## Input:

|Jefferson|
|Benton|
|Franklin|
|Faulkner|
|Madison|
|Garland|
|Poinsett|
|Craighead|
|Crawford|
|Lonoke|
|Lincoln|
|Pulaski|
|Crittenden|
|Miller|
|Cleveland|


## Output:

{"ERROR": "99999"}


------

## Input:

|2|
|4|
|1|
|6|
|29|


## Output:

{"ERROR": "$129.00"}

------

## Input:


|$70,000|
|$40,000|
|$90,000|
|$80,000|
|$60,000|
|$100,000|
|$130,000|
|$150,000|
|$50,000|
|$120,000|
|$160,000|
|$170,000|
|$110,000|
|$30,000|
|$10,000|
|$20,000|


## Output:

{"ERROR": "+1 800-425-1829"}



------

## Input:


|James Smith|
|Chris White|
|Jane Doe|
|Bill Gates|
|Steve Jobs|

## Output:

{"ERROR": "***"}


------

## Input:

|Labrador Retriever|
|French Bulldog|
|Golden Retriever|
|Poodle|
|German Shepherds|


## Output:

{"ERROR": "---"}

------

## Input:

|(41) 9635-0575|
|(47) 9285-3910|
|(15) 6518-6603|
|(91) 2727-6856|
|(61) 4425-1329|
|(78) 4464-7756|
|(23) 1443-9130|
|(94) 6570-4540|
|(54) 4294-8441|
|(62) 4022-2429|
|(29) 3528-8592|
|(72) 4078-7452|
|(12) 8805-7156|


## Output:

{"ERROR": "?"}

------

## Input:

|#ffd66a|
|#fbc527|
|#ff9212|


## Output:

{"ERROR": "2025"}

------

## Input:

|$100,000 to $250,000|
|$60,000 to $80,000|
|$80,000 to $100,000|
|$40,000 to $60,000|
|$20,000 to $40,000|
|less than $20,000|
|more than $250,000|


## Output:

{"ERROR": "-"}

------

## Input:

|108 lakeside court|
|2947 vine lane|
|620 woodside ct.|
|9539 glenside dr|
|101 candy rd.|
|6369 ellis street|
|9495 limewood place|
|5980 icicle circle|


## Output:

{"ERROR": "RGB(255, 87, 51)"}

------

## Input:

|1899-12-30 10:00:00.000|
|1899-12-30 14:00:00.000|
|1899-12-30 08:00:00.000|
|1899-12-30 12:00:00.000|
|1899-12-30 09:00:00.000|


## Output:

{"ERROR": "MD-192038"}

------

## Input:

|2017-wk19|
|2017-wk20|
|2017-wk21|
|2017-wk23|
|2017-wk24|
|2017-wk25|
|2017-wk26|
|2017-wk28|
|2017-wk29|
|2017-wk30|
|2017-wk31|


## Output:

{"ERROR": "g79"}

------

## Input:

|lonnie brien pol / lonnie.b.pol2@uscg.mil|
|shirley kraft / shirley.kraft@bpd.treas.gov|
|paulette anne swann / paulette.a.swann@uscg.mil|
|nekiesha michel bone-williams / nekiesha.m.edler@uscg.mil|
|alyssa chevalier / alyssa.chevalier@bpd.treas.gov|
|jeff hoge / jeffrey.hoge@fms.treas.gov|
|william stimmel / william.stimmel1@dhs.gov|
|james d. rapley / james.rapley@dhs.gov|
|/ kelly.rapley@dhs.gov|

## Output:

{"ERROR": "[4.72|2022-12-23 00:00:00|2022-12-23 00:00:00|Delivery]"}

------

Now given the input column below:

## Input:

|2012-2013|
|2011-2012|
|2010-2011|
|2009-2010|
|2008-09|
|2007-08|
|2006-07|
|2005-06|
|2004-05|
|2003-04|
|2002-03|
|2001-02|
|2000-01|
|1999-00|
|1998-99|
|1997-98|
|1996-97|
|1995-96|
|1994-95|
|1993-94|
|1992-93|
|1991-92|
|1990-91|
|1989-90|
|1988-89|
|1987-88|


Please brainstorm an **ERROR** cell <CELL>  **NOT** compatible with the <Column>. 

**DO** generate <CELL> using realistic strings
** NEVER ** generate fake <CELL> like "123 Main Street".
** NEVER ** generate fake <CELL> like "123456789"
** NEVER ** generate fake <CELL> like "12345"
** NEVER ** generate fake <CELL> like "ABC"
** NEVER ** generate fake <CELL> like "ABCD"
** NEVER ** generate fake <CELL> like "john.doe@example.com"

## Output:

{"ERROR": "2022-wk23"}

==> sections/Prompts/error_detection_validation.tex <==
# Task Description: The table column below is a high-quality real data column. In the unlikely event that you see any one cell that is clearly a data error, either because the cell is a typo/misspelling (e.g., Mississipi that is a misspelling of Mississippi), or because it is a semantic outlier that does not fit in the context of this column (e.g., a city name mixed in a column with country names, etc.), please point it out.

*** Please be aware that cell values that appear unusual are often NOT ERRORS, such as code values (e.g., "mdl-1023"), abbreviations (e.g., "MDX"), out-of-vocabulary words (e.g., foreign languages, or properietary terminologies), etc.. In all those cases, simply DO NOT make any prediction. Users will be very angry if they see incorrect predictions. ***
 
Please return {"obvious_error": "NULL"} if you believe the column is a high-quality column. Otherwise, please return any error cell you identified in JSON {"obvious_error": "<CELL>"}, ONLY IF you are ABSOLUTELY SURE that <CELL> is erroneous. We will manually verify and you will be punished if it turns out that <CELL> is not erroneous.

Input:
|Tortimer|
|Bowsser|
|Devan Shell|
|The Giant Turtle|
|Bowser|
|Tiptup|
|Shen-zin Su|
|Koopa Troopa|
|Valluta|
|Ghido|
|Bentley|


*** Please be aware that cell values that appear unusual are often NOT ERRORS, such as code values (e.g., "mdl-1023"), abbreviations (e.g., "MDX"), out-of-vocabulary words (e.g., foreign languages, or properietary terminologies), etc.. In all those cases, simply DO NOT make any prediction. Users will be very angry if they see incorrect predictions. ***
 
Please return {"obvious_error": "NULL"} if you believe the column is a high-quality column. Otherwise, please return any error cell you identified in JSON {"obvious_error": "<CELL>"}, ONLY IF you are ABSOLUTELY SURE that <CELL> is erroneous. We will manually verify and you will be punished if it turns out that <CELL> is not erroneous.

Output:

{"obvious_error": "NULL"}

==> sections/Prompts/r2r_sql_generation.tex <==
# Task description: The task of "program-by-example" or "transform data by-example", is to use a few given example output values in the new "DERIVED_COLUMN", to infer the underlying transformation program that was used to derive the given output values in the "DERIVED_COLUMN". This is also known as program-synthesis or program-by-example in the research literature.
 
Given the **Input table** shown below, we want to perform data transformations on this Input Table, to produce a **Desired Output Table**, with the new "DERIVED_COLUMN" shown as the rightmost column of the **Desired Output Table**.
 
Please inspect the given output examples in the "DERIVED_COLUMN" of the **Desired Output Table**, to identify the transformation program that can be used to produce the "DERIVED_COLUMN" using columns in the **Input table**. Please generate SQL code for the transformation that can execute on the **Input table**, to produce an output column that can exactly match the given output examples in the "DERIVED_COLUMN".
 
Please pay close attention to the format and the details of the given output examples in the "DERIVED_COLUMN", to make sure that your code will generate output values exactly matching the given examples, in terms of style, format, and casing.

For numerical computation, please use SQL Decimal class to avoid floating point precision issues, so always do "CAST(<computation> AS DECIMAL) AS DERIVED_COLUMN" if numbers are involved.

Also, to perform string concatenation in SQL using "||", always remember to cast both sides of "||" from number to string before performing concatenation, so always do "CAST(CAST(<computation> AS DECIMAL) AS TEXT) || "some string"", before you return your results.

Please do not use CASE statements, or anything that is like CASE/IF/ELSE, to hard code your transformation program (e.g., if row id == 1, return output-value-1, etc.). Please produce transformation programs that can *generalize* to new data rows from the same table, that are not shown below in the interest of space.

Your SQL code should always generate your target column in a column named "DERIVED_COLUMN" in your final result. You can assume that your SQL code will be executed on a SQLite3 database and on a table called "table".

No explanation, Return the final result as a markdown code block, as ```sql<SQL CODE>```.

**Input table:**
|MergedColumn|
|---|
|WR UFA Tennessee Titans|
|LB UFA Saskatchewan Roughriders (CFL)|
|LS UFA Omaha Nighthawks (UFL)|


**Desired Output Table:**
|MergedColumn|DERIVED_COLUMN|
|---|---|
|WR UFA Tennessee Titans|WR UFA Tennessee Titans|
|LB UFA Saskatchewan Roughriders (CFL)|LB UFA Saskatchewan Roughriders CFL|
|LS UFA Omaha Nighthawks (UFL)|LS UFA Omaha Nighthawks UFL|


No explanation, Return the final result as a markdown code block, as ```sql<SQL CODE>```.
Output:

```sql
SELECT 
    MergedColumn, 
    REPLACE(MergedColumn, ' (', ' ') AS DERIVED_COLUMN
FROM 
    table;
```

==> sections/Prompts/schema_matching_generation.tex <==
## Instruction:
Given the Table A shown below, please generate a new table Table B, so that *some* (but not all) of the generated columns in Table B can "map" to *some* (but not all) of columns in Table A, in the sense that they will refer to the same semantic concepts, such that they can "map" to each other.

When you generate new column names in Table B, please make sure that the new column names are different from the original column names in Table A.

When you generate new data values in Table B, please also make sure that you generate new data values not found in Table A.

After you generate Table B, please show how columns in Table A can map to columns in Table B. For each column in Table A, specify the corresponding column in Table B. If a column in A has no corresponding column in Table B, you can map it to None. Represent each column mapping using a pair of column headers in a list, i.e., [Table A Column, Table B column or None]. Provide the mapping for each column in Table A and return all mappings in a list. Return the final result as JSON in the format {"column_mappings": "<a list of column pairs>"}.

## Input:

Table A:
|Material collected|Pages|Publication Date|
|---|---|---|
|NYX #1-7|208|July 2011|
|NYX #1-7 & NYX: NO WAY HOME #1-6|392|July 2016|
|NYX #1-7 and X-23 Vol. 1, #1-6|352|November 2005|
|X-23 and the unrelated Firestar, Lady Deadpool, Namora, Valkyrie, Rescue, Sif, Spitfire, Galacta, Women of Marvel #1-2|352|February 2011|
|X-23 Vol. 1 #1-6|144|April 2006|
|X-23: Target X #1-6|160|August 2007|
|X-23 vol. 2 #1-6 and material from All-New Wolverine Saga|152|November 2011|
|Daken: Dark Wolverine #5-9, X-23 (Vol. 2) #7-9 And Material From Wolverine: Road To Hell.|200|February 2012|
|X-23 vol. 2 #10-16|152|July 25, 2012|
|X-23 vol. 2 #17-21|112|December 2012|


Please first return Table B in markdown format.
 
Please then return the column mapping result between Table A and Table B, using the following JSON format {"column_mappings": "<a list of column pairs>"}.

## Output:

Table B:
|Collected Material|Total Pages|Publishing Date|
|---|---|---|
|X-23 #1-7|215|August 2010|
|X-23: NO WAY HOME #1-6|380|June 2015|
|X-23 #1-7 and X-24 Vol. 1, #1-6|345|October 2004|
|X-24 and the unrelated Firestar, Lady Deadpool, Namora, Valkyrie, Rescue, Sif, Spitfire, Galacta, Women of Marvel #1-2|345|March 2010|
|X-23 Vol. 1 #1-6|140|May 2005|
|X-23: Target X #1-6|155|July 2006|
|X-24 vol. 2 #1-6 and material from All-New Wolverine Saga|148|October 2010|
|Daken: Dark Wolverine #5-9, X-24 (Vol. 2) #7-9 And Material From Wolverine: Road To Hell.|195|January 2011|
|X-24 vol. 2 #10-16|148|June 20, 2011|
|X-24 vol. 2 #17-21|110|November 2011|

## Column Mapping:
{"column_mappings": [["Material collected", "Collected Material"], ["Pages", "Total Pages"], ["Publication Date", "Publishing Date"]]}

==> sections/Prompts/schema_matching_validation.tex <==
# Task Description: Please identify the matching columns between Table A and Table B. For each column in Table A, specify the corresponding column in Table B. If a column in A has no corresponding column in Table B, you can map it to None. Represent each column mapping using a pair of column headers in a list, i.e., [Table A Column, Table B column or None]. Provide the mapping for each column in Table A and return all mappings in a list. Return the final result as JSON in the format {"column_mappings": "<a list of column pairs>"}.

## Input:
Table A:
|First elected|Councillor|Communities|Ward|
|---|---|---|---|
|2010|Doug Shipley|Little Lake, East Bayfield|3|
|2012|Arif Khan|Allandale, South Shore, Painswick North|8|
|2003|Barry Ward|Sunnidale, West Bayfield, Northwest|4|
|2014|Sergio Morales|Painswick South|9|
|2014|Rose Romita|Wellington, Queen's, City Centre, Lakeshore|2|
|2003|Michael Prowse|Ardagh|6|
|2006 (Councillor); 2010 (Mayor)|Jeff Lehman|At-large|Mayor|
|2010|Bonnie Ainsworth|Georgian Drive, Grove East, Codrington, North Shore|1|
|2010|Peter Silveira|Letitia Heights, Sandy Hollow, Edgehill Drive|5|
|2006 2016|John Brassard (until 2015) Andrew Prince (after 2016)|Holly|7|
|2014|Mike McCann|Innishore, Bayshore|10|


Table B:
|Year elected|Representative|District|Neighborhoods|
|---|---|---|---|
|2016|David Thompson|B|Hillcrest, Sunnyside|
|2012|Samantha Smith|A|Downtown, Riverdale|
|2010|Emily White|C|West End, Parkside|


Return the final result as JSON in the format {"column_mappings": "<a list of column pairs>"}.

## Output:

```json
{"column_mappings": [
  ["First elected", "Year elected"],
  ["Councillor", "Representative"],
  ["Communities", "Neighborhoods"],
  ["Ward", "None"]
]}
```
